Exploring Task Performance with Interpretable Models via Sparse Auto-Encoders

Large Language Models (LLMs) are traditionally viewed as black-box algorithms, therefore reducing trustworthiness and obscuring potential approaches to increasing performance on downstream tasks. In this work, we apply an effective LLM decomposition method using a dictionary-learning approach with sparse autoencoders. This helps extract monosemantic features from polysemantic LLM neurons. Remarkably, our work identifies model-internal misunderstanding, allowing the automatic reformulation of the prompts with additional annotations to improve the interpretation by LLMs. Moreover, this approach demonstrates a significant performance improvement in downstream tasks, such as mathematical reasoning and metaphor detection.

==> reviews.tex <==
\section{review 1}
Paper Summary:
This paper analyses the use of sparse auto-encoders (SAEs) to analyse the behaviour of LLMs when solving complex downstream tasks such as mathematical reasoning and metaphor detection and how that can be used to improve the model's performance on these downstream tasks. Specifically, the authors use SAE activations to identify whether the model might be misinterpreting the input and activating the wrong features (e.g., by parsing math formulas as code or URLs). When this happens, they use GPT4 to rephrase the input so to address the ambiguity issues.

The idea is super interesting -- however, I have a few significant concerns:

When and how often is the reformulation happening? If it's happening, e.g., 100% of the time, the takeaway message might be significantly different ("always reformulating instances with GPT4 into a simpler form always improves results"). However, if the ambiguity in the SAE features is a good proxy for predicting that the model will probably produce the wrong answer for a given instance and that reformulating these cases helps, the takeaway message is very different.
Here you assume you have GPT4 available -- can't you just use GPT4, then? What if you change GPT4 with something else? Can you use the same LLM to rephrase the inputs?
Summary Of Strengths:
Interesting idea
Significant improvements in downstream results
Summary Of Weaknesses:
When and how often is the reformulation happening? 100% of the times? 0.1%?
What if you use the same LLM, or some other LLM, in place of GPT4 for reformulating the instances?
Comments Suggestions And Typos:
If you provide more experimental details and analyses (see my "Weaknesses"), I'd be happy to revise my score

Confidence: 4 = Quite sure. I tried to check the important points carefully. It's unlikely, though conceivable, that I missed something that should affect my ratings.
Soundness: 3 = Acceptable: This study provides sufficient support for its major claims/arguments. Some minor points may need extra support or details.
Overall Assessment: 2 = Revisions Needed: This paper has some merit, but also significant flaws, and needs work before it would be of interest to the community.
Best Paper: No
Ethical Concerns:
There are no concerns with this submission

Reproducibility: 3 = They could reproduce the results with some difficulty. The settings of parameters are underspecified or subjectively determined, and/or the training/evaluation data are not widely available.
Datasets: 1 = No usable datasets submitted.
Software: 1 = No usable software released.
Knowledge Of Or Educated Guess At Author Identity: No
Knowledge Of Paper: After the review process started
Knowledge Of Paper Source: N/A, I do not know anything about the paper from outside sources
Impact Of Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources
Reviewer Certification: I certify that the review I entered accurately reflects my assessment of the work. If you used any type of automated tool to help you craft your review, I hereby certify that its use was restricted to improving grammar and style, and the substance of the review is either my own work or the work of an acknowledged secondary reviewer.


\section{review 2}

Paper Summary:
This paper uses sparse autoencoders and the auto-interpretability tool to understand the internal representations of LLMs. These explained features are then used to optimize the questions and improve smaller models' performance on difficult reasoning tasks.

Summary Of Strengths:
The refined questions can improve smaller models' performance on difficult reasoning tasks.
Summary Of Weaknesses:
It is not clear how the sparse autoencoder is utilized to improve models' abilities in difficult reasoning tasks after reading the introduction.
The technical contribution in this paper is limited. It is more like a work that combines existing techniques.
Mechanistic Interpretability is a broad area. The related work section spends a lot of space on explaining it rather than expanding more on technically related works. For example, works on superposition and polysemantic can be briefly mentioned instead of taking two paragraphs to explain them.
The auto-interpretability technique should be discussed in more details. For example, include its workflow and limitations in related work.
Why not use GPT to rephrase questions directly but using such a complicated process?
Comments Suggestions And Typos:
Can explaining LLMs be considered as one of the contributions of this work? Cunningham et al. 2023? have already applied it on LLMs.
The auto-interpretability technique is from Steven Bills et al. 2023.
Line 2330-236. It is not clear that if polysemanticity is the most critical reason for models' unsatisfactory performance on metaphor detection. Besides, does the problem in BERT and early-series GPTs still exist in large models now?
In Figure 2, step 2 is not included in Section 3.1.
Line 072-079 is difficult to follow, better reword it. I suppose the author is trying to say that features are more than number of neurons. If features are represented with their own individual dimension, the number of available dimensions(neurons) is not enough. As a result, features have to be represented by a combination of neurons.
It would be better to cite the original sparse autoencoder work Lee Sharkey et al. 2023
Confidence: 3 =  Pretty sure, but there's a chance I missed something. Although I have a good feel for this area in general, I did not carefully check the paper's details, e.g., the math or experimental design.
Soundness: 2.5
Overall Assessment: 1.5
Best Paper: No
Ethical Concerns:
There are no concerns with this submission

Needs Ethics Review: No
Reproducibility: 4 = They could mostly reproduce the results, but there may be some variation because of sample variance or minor variations in their interpretation of the protocol or method.
Datasets: 1 = No usable datasets submitted.
Software: 1 = No usable software released.
Knowledge Of Or Educated Guess At Author Identity: No
Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources
Knowledge Of Paper Source: N/A, I do not know anything about the paper from outside sources
Impact Of Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources
Reviewer Certification: I certify that the review I entered accurately reflects my assessment of the work. If you used any type of automated tool to help you craft your review, I hereby certify that its use was restricted to improving grammar and style, and the substance of the review is either my own work or the work of an acknowledged secondary reviewer.



\section{review 3}
Paper Summary:
The paper presents a novel approach to improving the interpretability and performance of LLMs by using sparse autoencoders to decompose model activations into monosemantic features. This decomposition aids in understanding and resolving model misunderstandings, thereby enhancing performance on tasks such as mathematical reasoning and metaphor detection.

Summary Of Strengths:
The use of sparse autoencoders to decompose LLM activations into monosemantic features is an application that addresses the challenge of polysemanticity in models. The proposed method demonstrates improvements in downstream tasks, particularly in complex reasoning and metaphor detection.

Summary Of Weaknesses:
The paper does not include comparative experimant with other methods that utilize sparse autoencoders [1,2,3]. In the realm of mathematical tasks, several approaches achieve improved performance without incurring fine-tuning costs, such as self-consistency [4] and proxy-tuning [5]. Additionally, supervised fine-tuning methods like chain-of-thought prompting [6] and teacher-student frameworks [7] have been effective in solving math problems. The paper lacks comparative experiments to demonstrate its effectiveness relative to these established methods.
[1] Rajamanoharan, Senthooran, et al. "Improving dictionary learning with gated sparse autoencoders." arXiv preprint arXiv:2404.16014 (2024).

[2] Lan, Michael, et al. "Sparse autoencoders reveal universal feature spaces across large language models." arXiv preprint arXiv:2410.06981 (2024).

[3] He, Zhengfu, et al. "Llama Scope: Extracting Millions of Features from Llama-3.1-8B with Sparse Autoencoders." arXiv preprint arXiv:2410.20526 (2024).

[4] Wang, Xuezhi, et al. "Self-consistency improves chain of thought reasoning in language models." arXiv preprint arXiv:2203.11171 (2022).

[5] Zhu, Wenhao, et al. "The Power of Question Translation Training in Multilingual Reasoning: Broadened Scope and Deepened Insights." arXiv preprint arXiv:2405.01345 (2024).

[6] Shi, Freda, et al. "Language models are multilingual chain-of-thought reasoners." arXiv preprint arXiv:2210.03057 (2022).

[7] Lu, Jianqiao, et al. "Yoda: Teacher-student progressive learning for language models." arXiv preprint arXiv:2401.15670 (2024).

Given that Anthropic has demonstrated a disconnect between feature activation context and resulting behavior [1], there is a need to ensure and explain how the sparse autoencoder accurately decomposes activations and overcomes this disconnect.
[1] Durmus, Esin, et al. "Evaluating feature steering: A case study in mitigating social biases, 2024." URL https://anthropic.com/research/evaluating-feature-steering.

The paper does not report the accuracy of the sparse autoencoder or detail how its performance was evaluated. It is crucial to provide metrics and assessments to validate the autoencoder's effectiveness in decomposing activations.

Why do you not use GPT-4 explain or rephrase the entire question directly?

There is an absence of ablation studies to determine the individual contributions of the decomposing activations and the rephrasing by GPT-4.

The experimental settings are not clearly described, including the training details for autoencoder, configurations, the parameters of autoencoder.

Is the sparse autoencoder model-agnostic or model-specific? Is the sparse autoencoder is layer-specific? Which layer does the autoencoder work on? Why select this layer? It needs further exploration.

Does this method also work with in-context learning?

There is no analysis of the additional costs associated with the proposed method, such as memory cost, computational resource cost, inference time cost, and other potential overheads.

Comments Suggestions And Typos:
see weakness

Confidence: 5 = Positive that my evaluation is correct. I read the paper very carefully and am familiar with related work.
Soundness: 2 = Poor: Some of the main claims/arguments are not sufficiently supported. There are major technical/methodological problems.
Overall Assessment: 2 = Revisions Needed: This paper has some merit, but also significant flaws, and needs work before it would be of interest to the community.
Best Paper: No
Ethical Concerns:
There are no concerns with this submission

Reproducibility: 3 = They could reproduce the results with some difficulty. The settings of parameters are underspecified or subjectively determined, and/or the training/evaluation data are not widely available.
Datasets: 3 = Potentially useful: Someone might find the new datasets useful for their work.
Software: 5 = Enabling: The newly released software should affect other people's choice of research or development projects to undertake.
Knowledge Of Or Educated Guess At Author Identity: No
Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources
Knowledge Of Paper Source: N/A, I do not know anything about the paper from outside sources
Impact Of Knowledge Of Paper: N/A, I do not know anything about the paper from outside sources
Reviewer Certification: I certify that the review I entered accurately reflects my assessment of the work. If you used any type of automated tool to help you craft your review, I hereby certify that its use was restricted to improving grammar and style, and the substance of the review is either my own work or the work of an acknowledged secondary reviewer.




1. Address Ambiguity in Reformulation and Its Frequency
Clearly explain when and how often input reformulation is triggered using GPT-4.
Quantify the percentage of instances where reformulation occurs.
Clearly explain the pipeline where ambiguity prediction via sparse autoencoders drives reformulation.
Add ablation studies comparing results with and without reformulation to highlight its contribution.

2. Generalize Reformulation Approach
Explore alternatives to GPT-4 for reformulation, such as using the same LLM or smaller LLMs.
Include comparative experiments to show whether similar improvements can be achieved with these alternatives.
Discuss the feasibility and limitations of relying on GPT-4 for reformulation in practical applications.

3. Improve Technical Details and Experimental Settings
Clearly describe the training details, configurations, and parameters of the sparse autoencoder.
Specify the autoencoder’s model-agnostic or model-specific nature, whether it is layer-specific, and why specific layers are selected.
Provide metrics to evaluate the performance of the sparsed autoencoder in decomposing activations.

4. Expand Related Work
Condense the discussion of mechanistic interpretability and polysemanticity to allocate space for more technically relevant works.
Discuss more limitations and workflows of auto-interpretability techniques, including those 【1，2】
【1】 Language models can explain neurons in language models
【2】Sparse Autoencoders Find Highly Interpretable Features in Language Models













